Non-collider searches for stable massive particles

The theoretical motivation for exotic stable massive particles (SMPs) and the results of SMP searches at non-collider facilities are reviewed. SMPs are defined such that they would be sufficiently long-lived so as to still exist in the cosmos either as Big Bang relics or secondary collision products, and sufficiently massive to be beyond the reach of any conceivable accelerator-based experiment. The discovery of SMPs would address a number of important questions in modern physics, such as the origin and composition of dark matter in the Universe and the unification of the fundamental forces. This review outlines the scenarios predicting SMPs and the techniques used at non-collider experiments to look for SMPs, eg in cosmic rays and bound in matter. The limits so far obtained on the fluxes and matter densities of SMPs which possess various detection-relevant properties such as electric and magnetic charge are given.

==> stringmonopole.tex <==
\subsection{Monopoles in Higher dimensions and in String theory}
There are a huge number of particles in higher dimensional theories which may posses magnetic charge.  It was pointed out by \cite{Sorkin:1983ns,Gross:1983hb} that monopoles in Kaluza Klein (KK) theories are expected to exist when the U(1) of electromagnetism is obtained by the symmetries of a closed loop in the compact dimensions.  This result is expected to hold in more realistic compactifications, although of course chirality remains a problem in such theories.

In String theory there are a variety of monopoles, in fact the aforementioned KK monopoles are also thought to be solutions of the wider theory \cite{Banks:1988rj}.  The same authors also pointed out that when one moves away from the self-dual compactifications radius where the symmetry between KK and winding modes leads to an enhanced SU(2) symmetry then the higgsing of the massless degrees of freedom at that point can give rise to monopoles exactly in the same manner as the 't Hooft-Polyakov monopole.

Five brands can couple to the magnetic potential associated with the anti-symmetric tensor field $B_{\mu\nu}$ and upon their dimensions lying along the six compact dimensions can appear as magnetic monopoles in the 3+1 dimensional theory \cite{Callan:1991ky,Gauntlett:1992nn}.  There are many such examples in different string theories with different compactifications and for each compactification upon a (typically complicated) compact manifold, there will be many different ways of wrapping extended magnetically charged objects resulting in point like monopoles in the 3+1D world.

In modern string theory, fundamental open strings have their ends attached to D-brands embedded in the higher dimensional space.  In some scenarios the gravity only part of the bulk can be pierced by lower-dimensional D-brane defects~\cite{Ellis:1998nz,Ellis:2008gg,Ellis:2004ay,Ellis:2005ib}. In our world, these particles would appear as point-like ``D-particles''~\cite{Ellis:1998nz,Ellis:2008gg,Ellis:2004ay,Ellis:2005ib,Shiu:2003ta}, non-perturbative stringy objects with masses of order m$_{D}\sim$ M$_{s}$/g$_{s}$, where g$_{s}$ is the string coupling.
The lightest D-particle (LDP) is stable, because it is the lightest state carrying its particular charge. Electrically and magnetically charged states are possible but normally the lightest state is assumed to be neutral to evade cosmological constraints (they are not observed in the same way magnetic monopoles are not observed) however there could be some aspect of cosmology which prevents them from being ruled out, such as inflation or a late time injection of entropy.  An important difference between the D-matter states and magnetic monopoles is that D-particles could have perturbative magnetic couplings.

The masses of all of these objects will be typically set by the string scale and/or the compactification scale of the compact space.  Since these are objects in which gauge fields can propagate, the constraints on their scale is set by the fact that 3+1D quantum field theory works well up to the multi-TeV energies of the LHC.  However typical theoretical descriptions usually set the compactification scale close to the GUT scale $10^{16}$ GeV although this can be reduced to lower energies, in particular when some of the extra dimensions are gravity only.  In those scenarios, the strongest constraint is the cosmology of the (now light) KK graviton modes associated with the large gravity only extra dimensions and the string scale and/or the inverse radius of the compact space (and hence the masses of the monopoles) can be brought close to the discovery reach of the LHC \cite{Fairbairn:2001ab}.




